SummAE: Zero-Shot Abstractive Text Summarization using Length-Agnostic Auto-Encoders

We propose an end-to-end neural model for zero-shot abstractive text summarization of paragraphs, and introduce a benchmark task, ROCSumm, based on ROCStories, a subset for which we collected human summaries. In this task, five-sentence stories (paragraphs) are summarized with one sentence, using human summaries only for evaluation. We show results for extractive and human baselines to demonstrate a large abstractive gap in performance. Our model, SummAE, consists of a denoising auto-encoder that embeds sentences and paragraphs in a common space, from which either can be decoded. Summaries for paragraphs are generated by decoding a sentence from the paragraph representations. We find that traditional sequence-to-sequence auto-encoders fail to produce good summaries and describe how specific architectural choices and pre-training techniques can significantly improve performance, outperforming extractive baselines. The data, training, evaluation code, and best model weights are open-sourced.

==> ack.tex <==
\section*{Acknowledgments}
\todo{Complete} Noah Fiedel for support;
Sammy Bengio and Arvind Neelakantan for reviewing.

==> bad_samples.tex <==

\begin{figure}[!h]
\small
\begin{mdframed}
\textbf{Story}\\
Vince was coming home from work one day. 
He began to pull up to his driveway and opened his garage door. 
Just as he parked and left his car, he heard a tremendous rumble.
Vince ran outside and his whole garage began to collapse. 
His car was crushed and Vince went inside out of extreme anger.
\\


\textbf{Human summaries}\\
1. Vince's car was crushed by his garage at home when he pulled into his driveway. \\
2. Vince's garage crushed his parked car. \\
3. Vince's collapsing garage crushed his car. \\


\textbf{Unsupervised abstractive summary (our model)}\\
Vince was driving home from work and saw his garage slamming. \\
\end{mdframed}

\normalsize

\caption{\todo{describe good samples}}
\label{fig:bad_samples}

\end{figure}


==> summary_with_reconstructions.tex <==
% Taken from https://cnsviewer.corp.google.com/cns/vz-d/home/peterjliu/sunsup/models/6048152/70/decodes/model.ckpt-62798.train.decode.txt

\begin{figure}[ht]
\small
\begin{mdframed}
\textbf{Story (paragraph) to summarize}\\
Tom woke up in the middle of the night.
His house alarm was going off.
Tom quickly checked to see what the problem was.
He wasn't able to find anything.He eventually reset the alarm and went back to sleep.
\\

\textbf{Reconstructed paragraph from autoencoder}\\
Tom woke up in the middle of the night.
His alarm was going off illegally.
He investigated what the time to see.
Tom checked the problem and was able to sleep.
He eventually realized he wasn't able to get back in a movie. \\
\\
\textbf{Reconstructed first sentence from autoencoder}\\
Tom woke up in the middle of the night.\\
\\
\textbf{Generated summary}\\
Tom woke up in the week and the car was broken.
\end{mdframed}

\normalsize

\caption{For a test example with an inaccurate generated summary, we show our autoencoder's reconstruction of the original story and the first sentence}
\label{fig:reconstructions}

\end{figure}

